Independent Emission and Absorption Abundances for Planetary Nebulae

Emission-line abundances have been uncertain for more than a decade due to unexplained discrepancies in the relative intensities of the forbidden lines and weak permitted recombination lines in planetary nebulae (PNe) and H II regions. The observed intensities of forbidden and recombination lines originating from the same parent ion differ from their theoretical values by factors of more than an order of magnitude in some of these nebulae. In this study we observe UV resonance line absorption in the central stars of PNe produced by the nebular gas, and from the same ions that emit optical forbidden lines. We then compare the derived absorption column densities with the emission measures determined from ground-based observations of the nebular forbidden lines. We find for our sample of PNe that the collisionally excited forbidden lines yield column densities that are in basic agreement with the column densities derived for the same ions from the UV absorption lines. A similar comparison involving recombination line column densities produces poorer agreement, although near the limits of the formal uncertainties of the analyses. An additional sample of objects with larger abundance discrepancy factors will need to be studied before a stronger statement can be made that recombination line abundances are not correct.

==> tab3-apj.tex <==
\begin{deluxetable*}{
c    %lambda
c    %logflambda
c    %species
c    %w_lambda
c    %logN
}
\tablecolumns{5}
\tablewidth{380pt}
\tablecaption{Equivalent Widths and Column Densities\label{tab3}}
\tablehead{
\colhead{$\lambda$\tablenotemark{a}~~~} & \colhead{$\log
f\lambda$\tablenotemark{a}~~~} & \colhead{Species~~~~~~} &
\colhead{$W_\lambda$\tablenotemark{b}} & \colhead{$\log N$\tablenotemark{b}}\\
\colhead{(\AA)} & \colhead{} & \colhead{} & \colhead{(m\AA)} & \colhead{$({\rm
cm}^{-2}$)}\\
}
\startdata
\cutinhead{{\bf He2-138}~~($v_*=-47\,{\rm km~s}^{-1};~-73 < v_{\rm PN} < -40\,{\rm
km~s}^{-1}$)}
1656.928 &  2.392 &C I &$    28.6\pm  4.4 $&  12.97 ($+ 0.07, -0.08$)\\
1560.309 &  2.082 &C I &$     2.6\pm  1.8 $&  12.25 ($+ 0.22, -0.47$)\\
1277.245 &  2.037 &C I &$    11.2\pm  1.8 $&  13.00 ($+ 0.07, -0.08$)\\
1548.204 &  2.468 &C IV &$   32.5\pm  4.2 $&  12.99 ($+ 0.06, -0.07$)\\
1550.781 &  2.167 &C IV &$   15.7\pm  4.0 $&  12.93 ($+ 0.10, -0.13$)\\
1550.781 &  2.167 &C IV &$   11.8\pm  2.6 $&  12.79 ($+ 0.09, -0.11$)\\
1304.858 &  1.795 &O I* &$   75.1\pm  1.2 $&  14.49 ($+ 0.05,
-0.05$)\tablenotemark{c}\\
1306.029 &  1.795 &O I** &$  64.9\pm  1.4 $&  14.38 ($+ 0.04,
-0.04$)\tablenotemark{c}\\
1306.029 &  1.795 &O I** &$  67.7\pm  2.2 $&  14.20 ($+ 0.08,
-0.10$)\tablenotemark{c}\\
1239.925 & -0.106 &Mg II &$   5.0\pm  1.3 $&  14.79 ($+ 0.10, -0.14$)\\
1239.925 & -0.106 &Mg II &$   4.2\pm  1.1 $&  14.72 ($+ 0.10, -0.14$)\\
1670.789 &  3.463 &Al II &$  91.4\pm 20.5 $&  12.69 ($+ 0.12,
-0.17$)\tablenotemark{c,d}\\
1304.370 &  2.052 &Si II &$  88.9\pm  1.0 $&  14.57 ($+ 0.04,
-0.05$)\tablenotemark{c,d}\\
1309.276\tablenotemark{e} &  2.052 &Si II* &$ 69.6\pm  2.3 $&  13.98 ($+ 0.02,
-0.02$)\tablenotemark{f}\\
1309.276\tablenotemark{e} &  2.052 &Si II* &$ 71.5\pm  2.4 $&  13.98 ($+ 0.02,
-0.02$)\tablenotemark{f}\\
1152.818 &  2.451 &P II &$   31.2\pm  3.8 $&  13.28 ($+ 0.09,
-0.11$)\tablenotemark{f}\\
1301.874 &  1.219 &P II &$    4.1\pm  1.1 $&  13.36 ($+ 0.11, -0.14$)\\
1153.995 &  2.331 &P II** & $11.2\pm  4.5 $&  12.83 ($+ 0.14, -0.22$)\\
1295.653 &  2.052 &S I &$     1.6\pm  1.6 $&  $<12.58$\\
1250.578 &  0.832 &S II &$   74.9\pm  2.0 $&  15.49 ($+ 0.08,
-0.09$)\tablenotemark{c}\\
1250.578 &  0.832 &S II &$   71.7\pm  1.2 $&  15.42 ($+ 0.10,
-0.14$)\tablenotemark{c}\\
1190.203 &  1.449 &S III &$  73.6\pm  2.3 $&  14.76 ($+ 0.12,
-0.16$)\tablenotemark{f}\\
1190.203 &  1.449 &S III &$  70.0\pm  1.6 $&  14.70 ($+ 0.02,
-0.02$)\tablenotemark{f}\\
1201.729 &  0.626 &S III**&$  16.3\pm  3.2$&  14.63 ($+ 0.08, -0.10$)\\
1197.184 &  2.414 &Mn II &$   9.4\pm  2.5 $&  12.66 ($+ 0.11, -0.15$)\\
1197.184 &  2.414 &Mn II &$  10.8\pm  2.2 $&  12.68 ($+ 0.08, -0.10$)\\
1199.391 &  2.308 &Mn II &$   6.2\pm  2.5 $&  12.53 ($+ 0.14, -0.22$)\\
1608.451 &  1.968 &Fe II &$  55.0\pm  2.3 $&  13.95 ($+ 0.03,
-0.04$)\tablenotemark{f}\\
1317.217 &  1.876 &Ni II &$   4.1\pm  1.3 $&  12.70 ($+ 0.12, -0.16$)\\
1317.217 &  1.876 &Ni II &$   5.3\pm  1.1 $&  12.81 ($+ 0.09, -0.11$)\\
1237.059 &  3.183 &Ge II &$   9.7\pm  1.3 $&  11.86 ($+ 0.06, -0.06$)\\
1237.059 &  3.183 &Ge II &$  11.6\pm  1.2 $&  11.94 ($+ 0.05, -0.05$)\\
1235.838 &  2.402 &Kr I &$    3.4\pm  1.9 $&  12.14 ($+ 0.18, -0.33$)\\
1235.838 &  2.402 &Kr I &$    4.6\pm  1.2 $&  12.25 ($+ 0.10, -0.14$)\\
\cutinhead{{\bf NGC~246}~~($v_*=-46\,{\rm km~s}^{-1};~-95 < v_{\rm PN} < -60\,{\rm
km~s}^{-1}$)}
1277.245 &  2.037 &C I &$     0.2\pm  1.0 $& $<12.29$\\
1334.532 &  2.234 &C II &$   12.9\pm  1.1 $&  12.84 ($+ 0.04, -0.04$)\\
1334.532 &  2.234 &C II &$   14.3\pm  1.0 $&  12.89 ($+ 0.03, -0.03$)\\
1335.708 &  2.234 &C II* &$  15.8\pm  1.0 $&  12.93 ($+ 0.03, -0.03$)\\
1199.550 &  2.199 &N I &$    -0.7\pm  1.0 $& $<12.04$\\
1302.169 &  1.796 &O I &$   4.3\pm  2.1 $&  12.80 ($+ 0.17,
-0.28$)\tablenotemark{g}\\
1302.169 &  1.796 &O I &$   0.6\pm  1.7 $& $<12.78$\tablenotemark{g}\\
1304.858 &  1.795 &O I* &$   -1.7\pm  1.3 $& $<12.44$\\
1260.422 &  3.171 &Si II &$   6.5\pm  2.6 $&  11.61 ($+ 0.14, -0.22$)\\
1264.738 &  3.125 &SiII* &$  -0.3\pm  1.0 $& $<11.14$\\
1206.500 &  3.293 &Si III &$ 49.7\pm  3.5 $&  12.52 ($+ 0.03, -0.03$)\\
1393.760 &  2.854 &Si IV &$ 145.1\pm  2.3 $&  13.50 ($+ 0.01,
-0.01$)\tablenotemark{f}\\
1402.773 &  2.552 &Si IV &$  97.6\pm  1.3 $&  13.51 ($+ 0.01, -0.01$)\\
1259.518 &  1.320 &S II &$    3.5\pm  2.2 $&  13.19 ($+ 0.20, -0.40$)\\
1190.203 &  1.449 &S III &$   3.4\pm  1.3 $&  13.08 ($+ 0.14, -0.21$)\\
1194.058 &  1.325 &S III* &$ -1.7\pm  2.5 $& $<13.32$\\
1317.217 &  1.876 &Ni II &$   2.1\pm  1.8 $&  12.40 ($+ 0.26, -0.71$)\\
1370.132 &  1.906 &Ni II &$  -0.6\pm  1.9 $& $<12.61$\\
\cutinhead{{\bf NGC~6543}~~($v_*=-66\,{\rm km~s}^{-1};~-103 < v_{\rm PN} <
-74\,{\rm km~s}^{-1}$)}
1277.245  &  2.037 &C I &$   1.1\pm  1.4 $& $<12.52$\\
1200.223  &  2.018 &N I &$   2.0\pm  1.7 $&  12.29 ($+ 0.25, -0.69$)\\
1304.858  &  1.795 &O I* &$   1.7\pm  1.3 $&  12.39 ($+ 0.25, -0.65$)\\
1306.029  &  1.795 &O I** &$  -0.3\pm  1.8 $& $<12.73$\\
1306.029  &  1.795 &O I** &$  -1.4\pm  1.3 $& $<12.47$\\
1670.789  &  3.463 &Al II &$   6.5\pm  4.5 $& 11.22 ($+0.22,-0.48$)\\  
1260.422  &  3.171 &Si II &$  85.9\pm  1.6 $&  13.11 ($+ 0.02,
-0.02$)\tablenotemark{c}\\
1526.707  &  2.307 &Si II &$  35.7\pm  2.0 $& 13.23 ($+0.03,-0.03$)\\ 
1304.370  &  2.052 &Si II &$  19.8\pm  1.4 $&  13.25 ($+ 0.03, -0.03$)\\
1264.738  &  3.125 &Si II* &$  88.8\pm  0.9 $&  13.17 ($+ 0.02,
-0.02$)\tablenotemark{c}\\
1533.432  &  2.307 &Si II* &$  43.5\pm  2.9 $& 13.33 ($+0.03,-0.03$)\\ 
1265.002  &  2.171 &Si II* &$  33.2\pm  1.5 $&  13.39 ($+ 0.02, -0.02$)\\
1309.276  &  2.052 &Si II* &$  22.6\pm  1.0 $&  13.31 ($+ 0.02, -0.02$)\\
1152.818  &  2.451 &P II &$   5.8\pm  6.2 $& $<12.81$\\
1259.518  &  1.320 &S II &$   9.6\pm  2.4 $&  13.65 ($+ 0.10, -0.12$)\\
1253.805  &  1.136 &S II &$   6.3\pm  1.3 $&  13.64 ($+ 0.08, -0.10$)\\
1190.203  &  1.449 &S III &$  93.2\pm  1.4 $&  14.92 ($+ 0.29,
-1.33$)\tablenotemark{c}\\
1194.058  &  1.325 &S III* &$  87.2\pm  1.7 $&  14.96 ($+ 0.02,
-0.03$)\tablenotemark{f}\\
1194.058  &  1.325 &S III* &$  86.5\pm  1.6 $&  14.95 ($+ 0.02,
-0.02$)\tablenotemark{f}\\
1197.184  &  2.414 &Mn II &$   1.3\pm  2.1 $& $<12.32$\\
1199.391  &  2.308 &Mn II &$   0.2\pm  2.2 $& $<12.38$\\
1608.451  &  1.968 &Fe II &$   0.1\pm  4.0 $& $<12.84$\\   
1317.217  &  1.876 &Ni II &$  -0.7\pm  1.6 $& $<12.56$\\
1370.132  &  1.906 &Ni II &$  -1.2\pm  2.2 $& $<12.64$\\
%\tablebreak
\cutinhead{{\bf Tc 1}~~($v_*=-83\,{\rm km~s}^{-1};~-128 < v_{\rm PN} < -86\,{\rm
km~s}^{-1}$)}
1560.309  &  2.082 &C I &$  -3.2\pm  4.1 $& $<12.65$\\
1277.245  &  2.037 &C I &$  -1.9\pm  2.4 $& $<12.54$\\
1199.550  &  2.199 &N I &$  -2.1\pm  3.1 $& $<12.53$\\
1302.169  &  1.796 &O I &$  27.1\pm  2.4 $&  13.63 ($+ 0.04,
-0.04$)\tablenotemark{h}\\
1306.029  &  1.795 &O I** &$   0.5\pm  2.0 $& $<12.83$\\
1239.925  & -0.106 &Mg II &$   0.2\pm  3.2 $& $<14.94$\\
1239.925  & -0.106 &Mg II &$   7.2\pm  3.8 $&  14.94 ($+ 0.18, -0.32$)\\
1670.787  &  3.463 &Al II &$  74.8\pm 22.9 $&  12.34 ($+ 0.12, -0.16$)\\
1260.422  &  3.171 &Si II &$ 110.7\pm  2.1 $&  13.22 ($+ 0.02,
-0.02$)\tablenotemark{c,d}\\
1193.290  &  2.842 &Si II &$  66.9\pm  3.7 $&  13.17 ($+ 0.03, -0.03$)\\
1190.416  &  2.541 &Si II &$  38.1\pm  4.4 $&  13.15 ($+ 0.05, -0.05$)\\
1304.370  &  2.052 &Si II &$  22.3\pm  1.2 $&  13.29 ($+ 0.02, -0.03$)\\
1264.738  &  3.125 &Si II* &$  99.8\pm  1.7 $&  13.18 ($+ 0.02,
-0.02$)\tablenotemark{c}\\
1265.002  &  2.171 &Si II* &$  22.9\pm  2.4 $&  13.20 ($+ 0.04, -0.05$)\\
1309.276  &  2.052 &Si II* &$  22.8\pm  1.7 $&  13.29 ($+ 0.03, -0.03$)\\
1152.818  &  2.451 &P II &$   7.3\pm  6.9 $&  12.52 ($+ 0.25, -0.66$)\\
1259.518  &  1.320 &S II &$  10.3\pm  2.0 $&  13.67 ($+ 0.08, -0.09$)\\
1190.203  &  1.449 &S III &$  79.9\pm  2.6 $&  14.65 ($+ 0.02, -0.02$)\\
1194.058  &  1.325 &S III* &$  49.5\pm  5.6 $&  14.46 ($+ 0.05, -0.06$)\\
1194.058  &  1.325 &S III* &$  48.4\pm  6.2 $&  14.46 ($+ 0.06, -0.07$)\\
1197.184  &  2.414 &Mn II &$  25.8\pm  4.8 $&  13.06 ($+ 0.08, -0.09$)\\
1197.184  &  2.414 &Mn II &$  25.9\pm  2.9 $&  13.05 ($+ 0.05, -0.05$)\\
1608.451  &  1.968 &Fe II &$  -2.9\pm  8.5 $& $<13.12$\\
1317.217  &  1.876 &Ni II &$   0.4\pm  1.4 $& $<12.60$\\
1237.059  &  3.183 &Ge II &$  -5.3\pm  3.2 $& $<11.43$\\
1237.059  &  3.183 &Ge II &$  -2.4\pm  3.8 $& $<11.63$\\
1235.838  &  2.402 &Kr I &$   9.0\pm  2.6 $&  12.53 ($+ 0.11, -0.15$)\\
\enddata

\tablenotetext{a}{Wavelengths and line strengths from
\citet{Mo00,Mo03}, except for the $f$-values of \ion{Ni}{2}, for which
we have adopted the values measured by \citet{JT01}.  Transitions for
individual species are arranged according to decreasing line strength.
This was done in order to make it easy to identify trends (strong
lines indicating smaller $N$ than weak ones) that signify possible
unresolved saturated components that could lead to underestimates of
column density using the AOD method \citep{SS91,Je96}.  Duplicate
entries signify independent measurements made in different echelle
orders.}
%
% Note "b" below is referenced in the text.  If it's changed, be sure
% to also change the text accordingly.
%
\tablenotetext{b}{{Listed} errors represent $\pm 1\sigma$ deviations and
include uncertainties caused by both photoevent statistical fluctuations
and continuum uncertainties, combined in quadrature.  When a measurement
of $W_\lambda$ yields a value that is below the calculated $1\sigma$
error in $W_\lambda$, we state the formal measurement of $W_\lambda$ and
its error, but then we follow with an evaluation of a $2\sigma$ upper
confidence bound for the real $W_\lambda$ using the method of
\citet{Ma92} for interpreting marginal detections (or nondetections) of
quantities that are known not to ever be negative.  The listed upper
limit for $N$ is calculated from this $W_\lambda$ limit using the
formula for weak lines (i.e., the linear part of the curve of
growth).}
%
\tablenotetext{c}{The line is strongly saturated (central optical depth
$\tau_0 \gtrsim 4$), but without a flat bottom that would signify severe
saturation.  The formal errors listed here may not accurately reflect
the true errors.  In our apparent optical depth integrations, occasional
deviations in $\tau_a(v)$ that exceeded 5.0 were simply set to equal to
5.0.}
%
\tablenotetext{d}{The right-hand portion of the profile is partly
blended with the left-hand portion of the absorption arising from
foreground material in the general interstellar medium.  Thus, the
errors could be somewhat larger than those derived formally (and stated
here).}
%
\tablenotetext{e}{\ion{Si}{2}* was also recorded at 1533.4$\,$\AA, but
this line is strong enough to have a small portion of its profile
strongly saturated.  Since our recording of the 1309.3$\,$\AA\ feature
is of excellent quality (and appeared in two orders), we decided not
to measure the stronger line.}
%
\tablenotetext{f}{At the bottom of the line, the intensity relative to
the continuum is less than 0.15.  For our representative $S/N=20$ (at
the continuum), the approximation given in equation~\ref{eq2} starts
to become inaccurate.  For this reason, the upper bound for $\log N$
should be increased slightly beyond the value listed here.}
%
\tablenotetext{g}{Absorption by the 1301.874$\,$\AA\ transition of
\ion{P}{2} caused by foreground gas interferes with the \ion{O}{1}
feature.  However, we could compensate for this by dividing the
spectrum by the \ion{P}{2} profile at 1152.818$\,$\AA\ after its
strength had been reduced to reflect the fact that the
1301.874$\,$\AA\ line is weaker.  (All intensities in the strong
profile were taken to a power equal to the ratio of the lines' values
of $f\lambda$.)}
%
\tablenotetext{h}{The right-hand portion of this profile is partly
blended with the left-hand side of an absorption arising from the
1301.874$\,$\AA\ transition of \ion{P}{2} created by the foreground
gas.}
\end{deluxetable*}

